Language to Rewards for Robotic Skill Synthesis

Large language models (LLMs) have demonstrated exciting progress in acquiring diverse new capabilities through in-context learning, ranging from logical reasoning to code-writing. Robotics researchers have also explored using LLMs to advance the capabilities of robotic control. However, since low-level robot actions are hardware-dependent and underrepresented in LLM training corpora, existing efforts in applying LLMs to robotics have largely treated LLMs as semantic planners or relied on human-engineered control primitives to interface with the robot. On the other hand, reward functions are shown to be flexible representations that can be optimized for control policies to achieve diverse tasks, while their semantic richness makes them suitable to be specified by LLMs. In this work, we introduce a new paradigm that harnesses this realization by utilizing LLMs to define reward parameters that can be optimized and accomplish variety of robotic tasks. Using reward as the intermediate interface generated by LLMs, we can effectively bridge the gap between high-level language instructions or corrections to low-level robot actions. Meanwhile, combining this with a real-time optimizer, MuJoCo MPC, empowers an interactive behavior creation experience where users can immediately observe the results and provide feedback to the system. To systematically evaluate the performance of our proposed method, we designed a total of 17 tasks for a simulated quadruped robot and a dexterous manipulator robot. We demonstrate that our proposed method reliably tackles 90% of the designed tasks, while a baseline using primitive skills as the interface with Code-as-policies achieves 50% of the tasks. We further validated our method on a real robot arm where complex manipulation skills such as non-prehensile pushing emerge through our interactive system.

==> prompts/motion_descriptor_meta.tex <==
\begin{tcolorbox}[
    colframe=darkgray, % Dark grey frame color
    boxrule=0.2pt, % Frame thickness
    colback=lightgray!20, %
    arc=3pt, % Rounded corners
    fontupper=\small,
    breakable
    ]

\end{tcolorbox}

==> prompts/reward_coder_meta.tex <==
\begin{tcolorbox}[
    colframe=darkgray, % Dark grey frame color
    boxrule=0.2pt, % Frame thickness
    colback=lightgray!20, %
    arc=3pt, % Rounded corners
    fontupper=\small,
    breakable
    ]

\end{tcolorbox}

==> task_list.tex <==
% instruction only version
\begin{table}[ht]
\scriptsize
% 	\vspace{-0.2cm}
	\begin{center}
		\begin{tabular}{l|l}
			\toprule
                \textbf{Quadruped Task Instructions} & \textbf{Manipulation Task Instructions} \\
                \midrule
                It's early in the morning, make the robot head towards the sun. & Touch the \texttt{\{obj\}} \\
                \midrule
                It's late in the afternoon, make the robot head towards the sunset. & Lift the \texttt{\{obj\}} to \SI{0.5}{m} \\
                \midrule
                Sit down low to ground with torso flat.& Move the \texttt{\{obj\_a\}} to \texttt{\{obj\_b\}}\\
                \midrule
                I want the robot to roll by 180 degrees. & Place the \texttt{\{obj\}} upright\\
                \midrule
                Spin fast. & Flip the \texttt{\{obj\}} \\
                \midrule
                I want the robot to lift its front right paw in the air. & Lift \texttt{\{obj\_a\}} and \texttt{\{obj\_b\}} together.\\
                \midrule
                \makecell[l]{I want the robot to lift its front right paw in the air.\\Lift it even higher.} & Turn on the faucet.\\
                \midrule
                \makecell[l]{Lift front left paw.\\Good, now lift diagonal paw as well.\\Good, in addition I want the robot to spin fast.} & Open the drawer.\\
                \midrule
                Make the robot stand upright on two back feet like a human.\\
			\bottomrule
		\end{tabular}
	\end{center}
	\caption{List of tasks used in evaluation for the quadruped robot and dexterous manipulator robot.}
	\label{tab:quadruped_tasks}
% 	\vspace{-0.3cm}
\end{table}

% task + instruction version
% \begin{table}[ht]
% \scriptsize
% % 	\vspace{-0.2cm}
% 	\begin{center}
% 		\begin{tabular}{l|l}
% 			\toprule
%                 \textbf{Task and Instructions} & \textbf{Task and Instructions} \\
%                 \midrule
%                 Facing sunrise: It's early in the morning, make the robot head towards the sun. & Touch object with hand: Touch the \texttt{\{obj\}} \\
%                 \midrule
%                 Facing sunset: It's late in the afternoon, make the robot head towards the sunset. & Lift object: Lift the \texttt{\{obj\}} to \SI{0.5}{m} \\
%                 \midrule
%                 Sit down: Sit down low to ground with torso flat.& Move object: Move the \texttt{\{obj\_a\}} to \texttt{\{obj\_b\}}\\
%                 \midrule
%                 Roll Over: I want the robot to roll by 180 degrees. & Upright object: Place the \texttt{\{obj\}} upright\\
%                 \midrule
%                 Spin: Spin fast. & Flip object: Flip the \texttt{\{obj\}} \\
%                 \midrule
%                 Lift one paw: I want the robot to lift its front right paw in the air. & Lift two objects : Lift \texttt{\{obj\_a\}} and \texttt{\{obj\_b\}} together.\\
%                 \midrule
%                 Lift paw higher: \makecell[l]{I want the robot to lift its front right paw in the air.\\Lift it even higher.} & Turn on the faucet: Turn on the faucet.\\
%                 \midrule
%                 Spin with lifted paws: \makecell[l]{Lift front left paw.\\Good, now lift diagonal paw as well.\\Good, in addition I want the robot to spin fast.} & Open the drawer: Open the drawer.\\
%                 \midrule
%                 Stand up on two feet: Make the robot stand upright on two back feet like a human.\\
% 			\bottomrule
% 		\end{tabular}
% 	\end{center}
% 	\caption{List of tasks used in evaluation for the quadruped robot and dexterous manipulator robot.}
% 	\label{tab:quadruped_tasks}
% % 	\vspace{-0.3cm}
% \end{table}


% \begin{table}[ht]
% \scriptsize
% % 	\vspace{-0.2cm}
% 	\begin{center}
% 		\begin{tabular}{ll}
% 			\toprule
%                 \textbf{Task} & \textbf{Instructions} \\
%                 \midrule
%                 Touch object with hand & Touch the \texttt{\{obj\}} \\
%                 \midrule
%                 Lift object & Lift the \texttt{\{obj\}} to \SI{0.5}{m} \\
%                 \midrule
%                 Move object & Move the \texttt{\{obj\_a\}} to \texttt{\{obj\_b\}} \\
%                 \midrule
%                 Upright object & Place the \texttt{\{obj\}} upright \\
%                 \midrule
%                 Flip object & Flip the \texttt{\{obj\}} \\
%                 \midrule
%                 Lift two objects & Lift the \texttt{\{obj\_a\}} and \texttt{\{obj\_b\}} at the same time. \\
%                 \midrule
%                 Turn on the faucet & Turn on the faucet. \\
%                 \midrule
%                 Open the drawer & Open the drawer. \\
% 			\bottomrule
% 		\end{tabular}
% 	\end{center}
% 	\caption{List of tasks used in evaluation for the dexterous manipulation.}
% 	\label{tab:manipulation_tasks}
% % 	\vspace{-0.3cm}
% \end{table}

